DeCaf: A Causal Decoupling Framework for OOD Generalization on Node Classification

Graph Neural Networks (GNNs) are susceptible to distribution shifts, creating vulnerability and security issues in critical domains. There is a pressing need to enhance the generalizability of GNNs on out-of-distribution (OOD) test data. Existing methods that target learning an invariant (feature, structure)-label mapping often depend on oversimplified assumptions about the data generation process, which do not adequately reflect the actual dynamics of distribution shifts in graphs. In this paper, we introduce a more realistic graph data generation model using Structural Causal Models (SCMs), allowing us to redefine distribution shifts by pinpointing their origins within the generation process. Building on this, we propose a casual decoupling framework, DeCaf, that independently learns unbiased feature-label and structure-label mappings. We provide a detailed theoretical framework that shows how our approach can effectively mitigate the impact of various distribution shifts. We evaluate DeCaf across both real-world and synthetic datasets that demonstrate different patterns of shifts, confirming its efficacy in enhancing the generalizability of GNNs.

==> proof.tex <==
% \yue{is this a theorem or property?}
% \begin{theorem}
\begin{customthm}{4.1}
Consider $n$ nodes with $c$ classes, such that the class distribution of all nodes is represented by $\mathbf{p} =p_1, p_2, ..., p_c$, where  $\sum_{i=1}^{c} p_i = 1$. If these nodes are randomly partitioned into $n'$ clusters such that $n' = \lfloor \gamma \cdot n \rfloor$, $0<\gamma<1$ and the class label for each cluster is determined via majority voting. The class distribution of all the clusters is 
% \yue{why is there an expectation on $p'_1$?}
$\mathbf{p}' = p'_1, p'_2, ... , p'_c$ where $p'_i$ is computed as the ratio of clusters labeled as class $i$ and $\sum_{i=1}^{c} p'_i = 1$.
Let $k$ be one of the classes, and the rest of the class are balanced $p_1 =...= p_{k-1} = p_{k+1}=... = p_c$.
% \yue{if the values are determined by ratios, this is not majority voting, maybe jus say "ratios of nodes"?}
% via majority voting, then the resultant class distribution is given by $p' = \mathbb{E}[p'_1], p'_2, ... , p'_c$, \yue{where $\mathbb{E}[p'_1]$ is computed as the ratio of nodes belonging to class 1. } and $\sum_{i=1}^{c} p'_i = 1$. 
It holds that:

1. If $p_k=1/c$ and all classes are balanced $p_1 = p_2 = ... = p_c$, then $\mathbb{E}[p'_k] = p_k$.

2. 
% \yue{notation: $p_1$ or $p_k$?}
When $p_k<1/c$, $\mathbb{E}[p'_k]<p_k$, and 
% \yue{what is the following?do you mean $\mathbb{E}[\frac{p'_k}{p_k}]$ decreases as ...}\xx{fixed}
$\mathbb{E}[\frac{p'_k}{p_k}]$ decreases as $n'$ decreases. There exists a $p^\text{min}$ such that $0<p^\text{min}<1$, and when $p_k<p^\text{min}$, $\mathbb{E}[\frac{p'_k}{p_k}]$ decrease as $p_k$ decreases. 
% \yue{how did you do calculate $p'_i$? Does $p'$ have only one 1 value and the rest 0 ? why is $p_i < p'_i$ after majority voting?} 
% \xx{$\mathbb{E}[p'_1]$ is the ratio of class 1 after the coarsening. Maybe should be the expectation of $\mathbb{E}[p'_1]$ instead}
% \xx {if a class have the most nodes, it is the majority class; if 2 classes share the same number of most nodes, each class has 50\% of chance to be selected as the majority class}
\end{customthm}

\begin{proof}
We prove the theorem by deriving the value of $\mathbb{E}[p'_k]$. Since $\mathbb{E}[p'_k]$ is invariant to the order of the classes, for convenience, we consider $i=1$ without losing generability. The probability of the first class after the partitioning is:
\begin{align}
\mathbb{E}[p'_1] = \frac{1}{n'}\sum_{a=1}^{n-n'} \mathbb{E}[n_a] q (a, \mathbf{p}),
\end{align}

where $\mathbb{E}[n_a]$ is the expectation of the number of clusters containing $a$ nodes, and $q (a, \mathbf{p})$ is the probability that class 1 is the majority class in a cluster with size $a$.

\begin{property}
The expectation of the number of clusters containing $a$ node is 
\[ \mathbb{E}[n_a] = n' \times \binom{n-n'+1}{a-1} \left(\frac{1}{n'}\right)^{a-1} \left(1 - \frac{1}{n'}\right)^{n-n'-(a-1)} .\]
\end{property}

\begin{proof}
Define \(I_{j}\) to be the indicator random variable for the \(j^{th}\) cluster, such that:
\[ I_{j} = 
\begin{cases} 
1 & \text{if the } j^{th} \text{ cluster contains exactly } a \text{ samples,} \\
0 & \text{otherwise.}
\end{cases}
\]
We first compute the expected value of \(I_{j}\) for a single cluster. Let's calculate the probability that \(a-1\) out of the \(n-n'\) samples are allocated to the \(j^{th}\) cluster:

(a) There are \(\binom{n-n'}{a-1}\) ways to choose \(a-1\) samples from the \(n-n'\) remaining samples.

(b) The probability that each of these \(a-1\) samples is placed in the \(j^{th}\) cluster is \(\left(\frac{1}{n'}\right)^{a-1}\).

(c) The remaining \(n-n'-a +1\) samples from our original pool of \(n-n'\) should not be allocated to the \(j^{th}\) cluster. The probability that all of them avoid this cluster is \(\left(1 - \frac{1}{n'}\right)^{n-n'-(a-1)}\).

Thus, the probability that the \(j^{th}\) cluster contains exactly \(x\) samples is:


\begin{align} \mathbb{E}[I_{j}] = \binom{n-n'}{a-1} \left(\frac{1}{n'}\right)^{a-1} \left(1 - \frac{1}{n'}\right)^{n-n'-(a-1)}. \end{align}

The expected number of clusters out of all \( n' \) clusters that contain exactly \( a \) samples is:

\begin{align} \mathbb{E}[n_a] = \sum_{j=1}^{n'} \mathbb{E}[I_{j}]. \end{align}

Given that each \( I_j \) is identically distributed, we can simplify the sum:

\begin{align} \mathbb{E}[n_a] = n' \times \mathbb{E}[I_{j}]. \end{align}

Substituting the expression derived for \( \mathbb{E}[I_{j}] \) from step 2, we obtain:

\begin{align}
\mathbb{E}[n_a] = n' \times \binom{n-n'}{a-1} \left(\frac{1}{n'}\right)^{a-1} \left(1 - \frac{1}{n'}\right)^{n-n'-(a-1)}. \end{align}
\end{proof}

It is easy to show that when $p_1 = p_2 = ... = p_c$, it holds that $q (a, \mathbf{p}) = \frac{1}{c}$ since all classes are equivalent and have equal chances to be the majority class. Thus:
\begin{align}
\mathbb{E}[p'_1] &= \frac{1}{n'}\sum_{a=1}^{n'} \mathbb{E}[n_a] q (a, \mathbf{p})
   \\&= \frac{1}{n'}\sum_{a=1}^{n'} \mathbb{E}[n_a] \frac{1}{c}
   \\&= \frac{1}{n'}\sum_{a=1}^{n'} n' \times \binom{n-n'}{a-1} \left(\frac{1}{n'}\right)^{a-1} \left(1 - \frac{1}{n'}\right)^{n-n'-(a-1)} \frac{1}{c}
   \\&= \frac{1}{n'} n' \frac{1}{c}
   \\&= \frac{1}{c}.
\end{align}

To compute $q (a, \mathbf{p})$, we need to consider the situations in which class 1 is the exclusive majority class and the cases where class 1 ties with one or more other classes for having the most samples. In the second case, we roll a die to select the majority class from all the classes that have most samples. 

To start, we consider the situation when class 1 has the most nodes and no other classes tie with it. We enumerate all possible combinations of class assignments and calculate the probability of each.  
\begin{align}
q_{0} (a,\mathbf{p}) = \sum_{i_1=1}^{a} \sum_{i_2=0}^{i_1-1}...\sum_{i_c=0}^{i_1-1}\mathbbm{1}\{\sum_{k=1}^{c} i_k =a\} f(\mathbf{i}, a, \mathbf{p}),
\end{align}
where $\mathbf{i} = i_1, i_2...i_c$,  and
\begin{align}
 f(\mathbf{i}, a, \mathbf{p}) 
 &= \prod_{k=1}^{c} \binom{a-i_1...-i_k}{i_k}  p_{k}^{i_k} (1-p_k)^{a-i_1-...-i_k},  
\end{align}

and 
\begin{align}
   p_k =
    \begin{cases}
      p_1 & \text{if $k=1$}\\
      \frac{1-p_1}{c-1} & \text{otherwise}\\
    \end{cases} . 
\end{align}

We then consider the situation when class 1 ties with another class. We first select another class that ties in with class 1, and we enumerate the possibility of other classes. We multiply the whole term by $\frac{1}{2}$ as there is an equal chance to select either class as the majority class. 

\begin{align}
q_{1} (a,\mathbf{p}) = \frac{1}{2} \sum_{j_1=2}^{c} \left(\sum_{i_1=1}^{a}  \sum_{i_2=0}^{i_1-1}...\sum_{i_{j_1}=i_1}^{i_1}...\sum_{i_c=0}^{i_1-1}\mathbbm{1}\{\sum_{k=1}^{c} i_k =a\} f(\mathbf{i}, a, \mathbf{p}) \right) .
\end{align}

We extend the above equation to a general case where class 1 ties with k classes ($1\leq k \leq c-1$). Here we need to select k   classes that tie with class 1. Class 1 now shares a $\frac{1}{k+1}$ chance to be selected as the majority class with the selected $k$ classes.
% \yue{missing content in the sum; also, should the front $\frac{1}{2}$ be $\frac{1}{k}$}
\begin{align}
q_{k} (a,\mathbf{p}) = \frac{1}{k} \sum_{j_1=2}^{c-k+1}\sum_{j_2=j_1}^{c-k+2}...\sum_{j_k=j_{k-1}}^{c} \left( \sum_{i_1=1}^{a}  \sum_{i_2=0}^{i_1-1}...\sum_{i_{j_1}=i_1}^{i_1}...\sum_{i_{j_k}=i_1}^{i_1}...\sum_{i_c=0}^{i_1-1} \mathbbm{1}\{\sum_{k=1}^{c} i_k =a\} f(\mathbf{i}, a, \mathbf{p})\right) .
\end{align}

Finally, we combine all the cases, and the probability that class 1 is the majority class is:

\begin{align}
q (a, \mathbf{p}) = \sum_{k=0}^{c-1} q_k (a, \mathbf{p}).
\end{align}

The expectation of $\frac{p'_1}{p_1}$ is thus:
\begin{align}
\mathbb{E}[\frac{p'_1}{p_1}] =
\frac{1}{p_1} \frac{1}{n'}\sum_{a=1}^{n'} \mathbb{E}[n_a] q (a, \mathbf{p}).
\end{align}
% \yue{where did the $p_1$ go in the $\frac{1}{p_1}$?}

To study the behavior of $\mathbb{E}[\frac{p'_1}{p_1}]$ when $p_1$ changes, we derive the following derivative:
\begin{align}
\frac{d\mathbb{E}[\frac{p'_1}{p_1}]}{dp_1} &= 
\frac {d\frac{1}{p_1} \frac{1}{n'}\sum_{a=1}^{n'} \mathbb{E}[n_a] q (a, \mathbf{p})}{dp_1}\\
&=  \frac{1}{n'}\sum_{a=1}^{n'} \mathbb{E}[n_a] 
\frac{d\frac{q (a, \mathbf{p})}{p_1}}{dp_1},
\end{align}

where 
% \yue{missing content in the sum}
\begin{align}
\frac{d\frac{q (a, \mathbf{p})}{p_1}}{dp_1} &=  \sum_{k=0}^{c-1} \frac{d\frac{q_k (a, p)}{p_1}}{dp_1}\\
&= \frac{1}{2} \sum_{j_1=2}^{c-k+1}\sum_{j_2=j_1}^{c-k+2}...\sum_{j_k=j_{k-1}}^{c} \left( \sum_{i_1=1}^{a}  \sum_{i_2=0}^{i_1-1}...\sum_{i_{j_1}=i_1}^{i_1}...\sum_{i_{j_k}=i_1}^{i_1}...\sum_{i_c=0}^{i_1-1} \mathbbm{1}\{\sum_{k=1}^{c} i_k =a\} \frac{d\frac{f(\mathbf{i}, a, \mathbf{p})}{p_1}}{dp_1}\right).
\end{align}

To find $\frac{d\frac{f(\mathbf{i}, a, \mathbf{p})}{p_1}}{dp_1}$, we first separate the terms that are independent of $p_1$:
\begin{align}
 \frac{f(\mathbf{i}, a, \mathbf{p})  }{p_1}
 &= \frac{1}{p_1} \prod_{k=1}^{c} \binom{a-i_1...-i_k}{i_k}  p_{k}^{i_k} (1-p_k)^{a-i_1-...-i_k}\\
 &= \frac{1}{p_1}  \left( \prod_{k=1}^{c} \binom{a-i_1...-i_k}{i_k}\right) \prod_{k=1}^{c}  p_{k}^{i_k} (1-p_k)^{a-i_1-...-i_k} \\
  &= \left( \prod_{k=1}^{c} \binom{a-i_1...-i_k}{i_k} \right) p_{1}^{i_1-1} (1-p_{1})^{a-i_1}(\frac{1-p_1}{c-1})^{\sum_{k=2}^{c} i_k} (1-\frac{1-p_1}{c-1})^{\sum_{k=2}^{c} a-i_2...-i_k} \\
    &= u \cdot p_{1}^{i_1-1} (1-p_{1})^{a-i_1}(1-p_1)^{\sum_{k=2}^{c} i_k} (p_1+c-2)^{\sum_{k=2}^{c} a-i_2...-i_k} \\
    &= u \cdot p_{1}^{
    \overbrace{i_1-1}^{\theta}}
     \cdot(1-p_{1})^{\overbrace{a-i_1 + \sum_{k=2}^{c} i_k}^{\phi}}
     \cdot (p_1+c-2)^{\overbrace{\sum_{k=2}^{c} a-i_2...-i_k}^{\psi}} ,
\end{align}
where $u$ is independent of $p_1$
\begin{align}
u = \left( \prod_{k=1}^{c} \binom{a-i_1...-i_k}{i_k} \right) (\frac{1}{c-1})
^{\sum_{k=2}^{c} i_k + \sum_{k=2}^{c} {a-i_2...-i_k}}
\end{align}
% \yue{why does it become $q_1$?}
We observe that $\frac{f(\mathbf{i}, a, \mathbf{p})}{p_1}$ demonstrates different behaviors for $a=1$ and $a>1$ and discuss the two cases separately.

(1) When \emph{$a=1$}, it holds that $i_1=1$, $\theta=0$, $\phi=0$, and $\psi=0$:
\begin{align}
\frac{f(\mathbf{i}, a, \mathbf{p})  }{p_1} = 
 u \cdot p_{1}^{0}
    (1-p_{1})^{0}
    (p_1+c-2)^{0} = u.
\end{align}

In such case, $\frac{d \frac{f(\mathbf{i}, a, \mathbf{p})}{p_1}}{dp_1}$ is independent with $p_1$ and remain constant when $p_1$ changes.


(2) When \emph{$a>1$}, it holds that $i_1\leq1$, $\theta\geq0$, $\phi\geq0$, $\psi\geq0$, and $\theta+\phi >0$:


\begin{align}
    \frac{d \frac{f(\mathbf{i}, a, \mathbf{p})}{p_1}}{dp_1} &= u\cdot p^{\theta-1}(1-p)^{\phi-1}(p+c-2)^{\psi-1}\cdot v, 
\end{align}
where
\begin{align}
    v &= \theta (1-p)(p+c-2) + \psi p(1-p) - \phi p(p+c-2)\\
    & = (-\theta - \phi - \psi)p^2 + (\theta + \psi + (\phi-\theta)(c-2))p + \theta(c-2).
\end{align}




When $0<p_1<1$ and $u>0$, $\frac{d \frac{f(\mathbf{i}, a, \mathbf{p})}{p_1}}{dp_1}=0$ if and only if $v=0$, 
and the corresponding value of $p_1$ is:
\begin{align}
p_1^0 = \frac{-\left(\theta - \theta \cdot (c-2) + \phi - \psi \cdot n\right) - \sqrt{\Delta}}{2\left(-\theta - \phi - \psi\right)},
\end{align}
\begin{align}
p_1^1 = \frac{-\left(\theta - \theta \cdot (c-2) + \phi - \psi \cdot n\right) + \sqrt{\Delta}}{2\left(-\theta - \phi - \psi\right)},
\end{align}
where 
\begin{align}
\Delta = \left(\theta - \theta \cdot (c-2) + \phi - \psi \cdot (c-2)\right)^2 - 4\left(-\theta - \phi - \psi\right)\left(\theta \cdot (c-2)\right).
\end{align}

It is easy to show that $\Delta>0$, and since $(-\theta - \phi - \psi)<0$, $v$ is concave, $v>0$ when $p_1^1 < p < p_1^0$. 
Also, it is observed that when $p_1=0$, 
\begin{align}
    v = \theta (c-2) \geq 0;
\end{align}
when  $p_1=1$,
\begin{align}
    v = -\phi (c-1) < 0.
\end{align}

Thus it must be held that $0<p_1^0<1$ and $p_1^1\leq 0$, and for any  $(\mathbf{i}, a>1)$, there exist a $0<p_1(\mathbf{i}, a>1)^0<1$ such that when $p_1<p_1^0(\mathbf{i}, a>1)$, $\frac{d\frac{f(\mathbf{i}, a, \mathbf{p})}{p_1}}{dp_1}>0$. 
Let 
\begin{align}
p_1^\text{min} = \min_{\forall a \in \{2,...,n'\}, \mathbf{i} \in \mathbf{I} } p_1^0(\mathbf{i}, a),
\end{align}
where $\mathbf{I}$ is all possible $\mathbf{i}$,  then it holds that $0<p_1^\text{min}<1$, and when $p_1<p_1^\text{min}$, $\frac{d\frac{q (a, \mathbf{p})}{p_1}}{dp_1} > 0$.

Next, we show that $\mathbb{E}[\frac{p'_1}{p_1}]$ decreases as $n'$ decreases when $p_1<1/c$. We first rewrite  $\mathbb{E}[\frac{p'_1}{p_1}]$ as
\begin{align}
\mathbb{E}[\frac{p'_1}{p_1}] =& \frac{1}{p_1}\frac{1}{n'}\sum_{a=1}^{n'} \mathbb{E}[n_a] q (a, \mathbf{p}) \\
=& \frac{1}{p_1}\sum_{a=1}^{n'} \binom{n-n'}{a-1} \left(\frac{1}{n'}\right)^{a-1} \left(1 - \frac{1}{n'}\right)^{n-n'-(a-1)} q (a, \mathbf{p})
\end{align}

First, we show that $q (a, \mathbf{p})$ is smaller for larger $a$ when $p_1< 1/c$. The intuition is that when a new node is added to a cluster originally with $a-1$ nodes, the new node has a higher probability of being another class, and the likelihood of class 1 becoming the majority class decreases.

Next, we show that when $n'$ increases,  $\binom{n-n'}{a-1} \left(\frac{1}{n'}\right)^{a-1} \left(1 - \frac{1}{n'}\right)^{n-n'-(a-1)}$ becomes more left-skewed, that it gives a smaller value for large $a$. The intuition is that, as the value of $n'$ increases, the average cluster size is expected to decrease. As a result, a large $a$ becomes farther from the average cluster size, and the probability of a cluster having exactly $a$ nodes decreases, leading to a decrease in the ratio of clusters with size $a$. 

% the larger $n'$ is, the smaller the average cluster size would be, and the further $a$ is from the average cluster size, the smaller the probability that a cluster has $a$ nodes will be, and the ratio of clusters with size $a$ hereby decreases. 

With the above observations, it can be concluded that when $ p_1<1/c $, the value of $\mathbb{E}[\frac{p'_1}{p_1}]$ decreases as $n'$ decreases.
\end{proof}



% Given $ n $ nodes from $ c $ classes with class distribution $ p = p_1, p_2, ...,p_c $ (where $ p_1+p_2+... +p_c = 1 $) randomly partitioned into $ n' $ clusters, and the class label of each cluster is determined by majority voting. Let $p' = \mathbb{E}[p'_1], p'_2, ... ,p'_c (\mathbb{E}[p'_1]+p'_2+... +p'_c)$ be class distribution after the partitioning. If $p_1 = p_2 =...= p_c$, then $pi = p'_i, i\in {\{1,2,...,c\}}$; otherwise, for any class $i$ such that $p_i<\frac{1}{c}$, it holds that $p_i<p'_i$, and the smaller $p_i$ is, the smaller $\frac{p_i}{p'_i}$ will be. 

% Given $n$ nodes from $c$ classes with class distribution $p = p_1, p_2, ... ,p_c (p_1+p_2+... +p_c)$ randomly partitioned into $n'$ clusters, and the class label of each cluster is determined by majority voting. Let $p' = \mathbb{E}[p'_1], p'_2, ... ,p'_c (\mathbb{E}[p'_1]+p'_2+... +p'_c)$ be class distribution after the partitioning. Then the probability of the first class after the partitioning is:
% \begin{align}
% \mathbb{E}[p'_1] = \frac{1}{n'}\sum_{i=1}^{n'} \mathbb{E}[a_i] q (i, p),
% \end{align}
% where $\mathbb{E}[n_a]$ is the expectation of number of clusters containing $a$ node:
% \begin{align}
% \mathbb{E}[n_a] = n' \times \binom{n-n'}{a-1} \left(\frac{1}{n'}\right)^{a-1} \left(1 - \frac{1}{n'}\right)^{n-n'-(a-1)},
% \end{align}
% and $q (a, \mathbf{p})$ is the probability that class 1 is the majority class  
% in a cluster with size $a$. When $c=2$:
% \begin{align}
% q (a, \mathbf{p}) = \sum_{i=\lfloor a/2 \rfloor}{n} \binom{a}{i} p_{1}^{i} (1-p_1)^{a-i} + \mathbbm{1}\{a\%2==0\} \frac{1}{2} \binom{a}{a/2} p_{1}^{a/2} (1-p_1)^{a/2},
% \end{align}
% when $c=3$:
% \begin{align}
% q (a, \mathbf{p}) &= \sum_{i=\lfloor a/2 \rfloor}{n} \binom{a}{i} p_{1}^{i} (1-p_1)^{a-i}\\ &+  \sum_{i=\lfloor a/3 \rfloor+1}{\lfloor a/2 \rfloor} \binom{a-i}{j} p_{2}^{j} (1-p_2)^{a-i-j} \\&+ 
% \binom{a-i}{i} p_{2}^{i} (p_3)^{a-2i} +
% \binom{a-i}{i} p_{3}^{i} (p_2)^{a-2i} \\&+   
% \mathbbm{1}\{a\%3==0\}  \frac{1}{3} 
% \binom{a}{a/3} p_{1}^{a/3} (1-p_1)^{a/3},
% \end{align}

% Given \( n \) samples partitioned into \( n' \) clusters such that one cluster contains at least one sample, the expected number of clusters that contain exactly \( a \) samples is:

% \[ E(n_a) = n' \times \binom{n-n'}{a-1} \left(\frac{1}{n'}\right)^{a-1} \left(1 - \frac{1}{n'}\right)^{n-n'-(a-1)} \]

% **Proof**:

% 1. **Indicator Random Variables**: Define \(I_{j}\) to be the indicator random variable for the \(j^{th}\) cluster, such that:

% \[ I_{j} = 
% \begin{cases} 
% 1 & \text{if the } j^{th} \text{ cluster contains exactly } a \text{ samples,} \\
% 0 & \text{otherwise.}
% \end{cases}
% \]

% 2. **Probability Calculation for a Single Cluster**: We first compute the expected value of \(I_{j}\) for a single cluster.

% Let's calculate the probability that \(a-1\) out of the \(n-n'\) samples are allocated to the \(j^{th}\) cluster:

% (a) There are \(\binom{n-n'}{a-1}\) ways to choose \(a-1\) samples from the \(n-n'\) remaining samples.

% (b) The probability that each of these \(a-1\) samples is placed in the \(j^{th}\) cluster is \(\left(\frac{1}{n'}\right)^{a-1}\).

% (c) The remaining \(n-n'-a +1\) samples from our original pool of \(n-n'\) should not be allocated to the \(j^{th}\) cluster. The probability that all of them avoid this cluster is \(\left(1 - \frac{1}{n'}\right)^{n-n'-(a-1)}\).

% Thus, the probability that the \(j^{th}\) cluster contains exactly \(a\) samples is:

% \[ E(I_{j}) = \binom{n-n'}{a-1} \left(\frac{1}{n'}\right)^{a-1} \left(1 - \frac{1}{n'}\right)^{n-n'-(a-1)} \]

% 3. **Using Linearity of Expectation**: We wish to determine the expected number of clusters, out of all \( n' \) clusters, that contain exactly \( a \) samples:

% \[ E(n_a) = \sum_{j=1}^{n'} E(I_{j}) \]

% Given that each \( I_j \) is identically distributed, we can simplify the sum:

% \[ E(n_a) = n' \times E(I_{j}) \]

% Substituting the expression derived for \( E(I_{j}) \) from step 2, we obtain:

% \[ E(n_a) = n' \times \binom{n-n'}{a-1} \left(\frac{1}{n'}\right)^{a-1} \left(1 - \frac{1}{n'}\right)^{n-n'-(a-1)} \]

% This completes our proof. 

\begin{customobs}{4.1}
  Node Fidelity Preservation with buffer size $b$ can alleviate the declination of a minority class $k$ when $p_k$ decreases and $n'$ decreases, and prevent class $k$ from vanishing at small when $p_k$ is small.  
\end{customobs}

The mechanism of Node Fidelity Preservation is to ``hold'' $b$ clusters such that each cluster only has 1 node. We already show that when $a=1$, $\frac{q(a, \mathbf{p})}{q_1}$ is independent of $q_1$ and so $\mathbb{E}[p'_1] = p_1$. By doing so, we make sure that among the $b$ nodes, class 1 does not decline as $p_1$ or $n'$ decline. 

\begin{figure}
\centering
\begin{tabular}{cc}
  \includegraphics[width=50mm]{images/ratio_c_2.pdf}&\includegraphics[width=50mm]{images/p1_c_2.pdf}\\
  (a) $\mathbb{E}[\frac{p'_1}{p_1}]$ vs. $p_1$, $c=2$ & (b) ${\mathbb{E}[p'_1]}$ vs. $p_1$, $c=2$\\[2pt]
\includegraphics[width=50mm]{images/ratio_c_3.pdf}&\includegraphics[width=50mm]{images/p1_c_3.pdf}\\
(c) $\mathbb{E}[\frac{p'_1}{p_1}]$ vs. $p_1$, $c=3$ & (d) ${\mathbb{E}[p'_1]}$ vs. $p_1$, $c=3$\\[2pt]
\end{tabular}
\caption{ $\mathbb{E}[p'_1]$ and $\mathbb{E}[\frac{p'_1}{p_1}]$ against $p_1$ at different reduction rate $\gamma$ for $c=2$ and $c=3$. The dashed lines represent trends with Node Fidelity Preservation (NFP), and the solid lines represent trends without NFP. }
\label{fig::p1}
\end{figure}

We demonstrate the effect of Node Fidelity Preservation with examples. We assign $n=1000$, $c=2, 3$, and $b=\lfloor n'/5 \rfloor$. 
we plot change of $\mathbb{E}[\frac{p'_1}{p_1}]$ and $\mathbb{E}[p'_1]$ at different $n'$ and $p_1$ separately in Figure \ref{fig::p1}. We draw the trend with Node Fidelity Preservation (NFP) using dash lines and without NFP using solid lines. From the figure, we observe that without Node Fidelity Preservation being applied, the ratio $\mathbb{E}[\frac{p'_1}{p_1}]$ approaches zero when $n'$ is small, resulting in a vanishing minority class. The application of Node Fidelity Preservation prevents the ratio from approaching zero and makes sure class 1 won't disappear when $p_1$ is small.  



